Accurate Hellmann-Feynman forces from density functional calculations with augmented Gaussian basis sets

The Hellmann-Feynman (HF) theorem provides a way to compute forces directly from the electron density, enabling efficient force calculations for large systems through machine learning (ML) models for the electron density. The main issue holding back the general acceptance of the HF approach for atom-centered basis sets is the well-known Pulay force which, if naively discarded, typically constitutes an error upwards of 10 eV/Ang in forces. In this work, we demonstrate that if a suitably augmented Gaussian basis set is used for density functional calculations, the Pulay force can be suppressed and HF forces can be computed as accurately as analytical forces with state-of-the-art basis sets, allowing geometry optimization and molecular dynamics to be reliably performed with HF forces. Our results pave a clear path forwards for the accurate and efficient simulation of large systems using ML densities and the HF theorem.

==> analyze_geom.tex <==
\begin{table}
    \centering

    \begin{tabular}{|p{0.2\textwidth}|p{0.615\textwidth}|}
    \hline    System & \begin{tabular}{p{0.2\textwidth}|p{0.075\textwidth}|p{0.075\textwidth}|p{0.075\textwidth}|p{0.075\textwidth}}
    Optimization & $\Delta d_{avg}$ & $\Delta d_{max}$ & $\Delta \theta_{avg}$ & $\Delta \theta_{max}$ \\
    \end{tabular}\\
    \hline
    \hline
     water    &  \begin{tabular}{p{0.2\textwidth}|p{0.075\textwidth}|p{0.075\textwidth}|p{0.075\textwidth}|p{0.075\textwidth}}
    None & 1.26  & 3.24 & 4.34 & 4.34 \\
    $\sigma$DZHF $\vec{F}^{HF}$ & 0.06 & 0.06 & 0.16 & 0.16 \\
    $\sigma$DZHF $\vec{F}^{E}$ & 0.03 & 0.10 & 0.14 & 0.14 \\
     \end{tabular} \\
     \hline
     ammonia  & \begin{tabular}{p{0.2\textwidth}|p{0.075\textwidth}|p{0.075\textwidth}|p{0.075\textwidth}|p{0.075\textwidth}}
    None & 0.72  & 1.33 & 1.58 & 2.11 \\
    $\sigma$DZHF $\vec{F}^{HF}$ & 0.15 & 0.20 & 0.32 & 0.43 \\
    $\sigma$DZHF $\vec{F}^{E}$ & 0.14 & 0.21 & 0.30 & 0.40 \\
     \end{tabular} \\
    \hline
     ethane  & \begin{tabular}{p{0.2\textwidth}|p{0.075\textwidth}|p{0.075\textwidth}|p{0.075\textwidth}|p{0.075\textwidth}}
    None & 0.77  & 1.52 & 1.53 & 2.74 \\
    $\sigma$DZHF $\vec{F}^{HF}$ & 0.02 & 0.05 & 0.01 & 0.02 \\
    $\sigma$DZHF $\vec{F}^{E}$ & 0.01 & 0.02 & 0.01 & 0.01 \\
     \end{tabular} \\
    \hline
    acetylene  & \begin{tabular}{p{0.2\textwidth}|p{0.075\textwidth}|p{0.075\textwidth}|p{0.075\textwidth}|p{0.075\textwidth}}
    None & 3.57  & 6.01 & 0.00 & 0.00 \\
    $\sigma$DZHF $\vec{F}^{HF}$ & 0.01 & 0.01 & 0.00 & 0.00 \\
    $\sigma$DZHF $\vec{F}^{E}$ & 0.02 & 0.03 & 0.00 & 0.00 \\
     \end{tabular} \\
    \hline
    allene  & \begin{tabular}{p{0.2\textwidth}|p{0.075\textwidth}|p{0.075\textwidth}|p{0.075\textwidth}|p{0.075\textwidth}}
    None & 0.56  & 1.61 & 3.46 & 100. \\
    $\sigma$DZHF $\vec{F}^{HF}$ & 0.02 & 0.04 & 0.09 & 2.48 \\
    $\sigma$DZHF $\vec{F}^{E}$ & 0.02 & 0.02 & 0.04 & 0.55 \\
     \end{tabular} \\
    \hline
    methylamine  & \begin{tabular}{p{0.2\textwidth}|p{0.075\textwidth}|p{0.075\textwidth}|p{0.075\textwidth}|p{0.075\textwidth}}
    None & 1.20  & 2.10 & 0.68 & 2.31 \\
    $\sigma$DZHF $\vec{F}^{HF}$ & 0.04 & 0.12 & 0.05 & 0.30 \\
    $\sigma$DZHF $\vec{F}^{E}$ & 0.01 & 0.04 & 0.03 & 0.20 \\
     \end{tabular} \\
    \hline
    hydroxysulphane & \begin{tabular}{p{0.2\textwidth}|p{0.075\textwidth}|p{0.075\textwidth}|p{0.075\textwidth}|p{0.075\textwidth}}
    None & 3.67  & 8.05 & 7.85 & 13.1 \\
    $\sigma$DZHF $\vec{F}^{HF}$ & 0.16 & 0.33 & 0.36 & 0.83 \\
    $\sigma$DZHF $\vec{F}^{E}$ & 0.03 & 0.09 & 0.11 & 0.20 \\
     \end{tabular} \\
    \hline
    ethanol & \begin{tabular}{p{0.2\textwidth}|p{0.075\textwidth}|p{0.075\textwidth}|p{0.075\textwidth}|p{0.075\textwidth}}
    None & 1.45  & 5.41 & 3.30 & 13.0 \\
    $\sigma$DZHF $\vec{F}^{HF}$ & 0.05 & 0.25 & 0.05 & 0.23 \\
    $\sigma$DZHF $\vec{F}^{E}$ & 0.02 & 0.07 & 0.02 & 0.12 \\
     \end{tabular} \\
    \hline
      \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}


==> asDZ0HF.tex <==
basis =  {  !asDZ0HF
 S   H      2766.0000    401.7000     94.7500     27.7500      9.1680      2.5810      0.7886      0.2639      0.0948      0.0193
 c 1.10   0.2735117693D-04  0.1889730094D-03  0.1063272508D-02  0.3567855378D-02  0.1706323987D-01  0.7684443035D-01  0.2469054991D+00  0.4888400802D+00  0.3005854711D+00  0.1094293475D-01
 c 1.10   0.9503508614D-04  0.7347946061D-03  0.3637520418D-02  0.1550913637D-01  0.5442997913D-01  0.2906990580D+00  0.7873016767D+00 -0.2401105835D+00 -0.7049085465D+00 -0.5445913987D-01
 c 1.10   0.5210290799D-04  0.4154905838D-03  0.2070880984D-02  0.8877971993D-02  0.2978400271D-01  0.1559453149D+00  0.3936651531D+00 -0.6943193153D+00 -0.2875843874D+00  0.1139848883D+01
 c 1.10   0.8287958478D-05 -0.4677355999D-02 -0.7384059334D-02 -0.9393459457D-01 -0.4342408558D-01  0.1341275386D+01 -0.9283433145D+00 -0.1049381845D+01  0.1623357713D+01 -0.6883564320D+00
 P   H      2766.0000    401.7000     94.7500     27.7500      9.1680      2.5810      0.7886      0.2639      0.0948      0.0193
 c 1.10  -0.1624120862D-08  0.1061643854D-08  0.8506240353D-09 -0.1049378495D-07 -0.9195743460D-08  0.1317121456D+00  0.6002006498D+00  0.3938333261D+00  0.5811753100D-02 -0.2381922156D-07
 c 1.10   0.3599581129D-02  0.1126418706D-01  0.2435932983D-01  0.6626094112D-01  0.1105536032D+00  0.3398819543D+00  0.3884744658D+00 -0.4114482331D+00 -0.5103995335D+00 -0.2046330800D+00
 c 1.10   0.4264751120D-02  0.1251387659D-01  0.3408127076D-01  0.6596177232D-01  0.1514497536D+00  0.2857756696D+00  0.2258895532D+00 -0.8165975293D+00  0.3674641621D+00  0.7381242040D+00
 c 1.10  -0.1245785901D-01 -0.3294526297D-01 -0.8733089999D-01 -0.1659027183D+00 -0.4400035682D+00 -0.4534480227D+00  0.1013429496D+01 -0.5140936813D+00 -0.3839922742D+00  0.4690850256D+00
 D   H         2.5810      0.7886      0.2639      0.0948
 c 1.4   0.2644474169D+00  0.6661436239D+00  0.2528456500D+00  0.2234712397D-02
 S   C    178500.0000  26640.0000   6033.0000   1698.0000    548.6000    195.7000     75.8200     31.5200     13.5700      5.8950      2.5730      1.0510      0.4243      0.1681      0.0637      0.0800
 c 1.16   0.1119761967D-04  0.8787774344D-04  0.4648798746D-03  0.1980034352D-02  0.7256314010D-02  0.2339875686D-01  0.6472136200D-01  0.1505972453D+00  0.2876136986D+00  0.3702892471D+00  0.1999411768D+00  0.2754805959D-01  0.3475487459D-01  0.3071023656D-01  0.3811679996D-02 -0.2575613456D-06
 c 1.16   0.3221151218D-05  0.2498231010D-04  0.1327840875D-03  0.5648449043D-03  0.2080785693D-02  0.6746619812D-02  0.1905344528D-01  0.4603617676D-01  0.9666435715D-01  0.1574298368D+00  0.1439484593D+00 -0.1185001684D+00 -0.5162953333D+00 -0.4594845277D+00 -0.5709524852D-01  0.5402456652D-06
 c 1.16   0.2736772234D-05  0.2524952893D-04  0.1337890657D-03  0.5363345497D-03  0.2120819400D-02  0.6270870403D-02  0.2078376908D-01  0.4238655817D-01  0.1156720128D+00  0.1574823782D+00  0.3100318161D+00 -0.8382596379D+00 -0.9564408523D+00  0.1236105436D+01  0.2191722541D+00  0.3323819761D-06
 c 1.16  -0.1428708538D-05 -0.1828516716D-04 -0.8259775432D-04 -0.3758921093D-03 -0.1436262744D-02 -0.3394008459D-02 -0.1586735900D-01 -0.2076967166D-01 -0.9499636215D-01 -0.9124862267D-01 -0.3291980125D+00  0.1323828452D+01 -0.2302985639D+00 -0.2061628090D+01  0.1919760341D+01  0.3116115036D-06
 c 1.16  -0.1764145979D-02 -0.3514273512D-02  0.1155264975D-01 -0.2420049537D-01  0.7551847916D-01 -0.1054280291D+00  0.3349301267D+00 -0.3305714613D+00  0.8740469553D+00 -0.1823490345D+01  0.6274825229D+00  0.2386019059D+01 -0.3323828286D+01  0.1625839420D+00 -0.7981991580D+01  0.9004501168D+01
 c 1.16  -0.1781111829D-02 -0.1300870191D-02  0.6463334298D-02 -0.9312253640D-03  0.4812808671D-01  0.1106438496D-01  0.2854719747D+00  0.1970120229D+00  0.8293399716D+00 -0.5406775811D+00 -0.1719271123D+01  0.1400234031D+01  0.5863242208D+00 -0.2210785297D+01 -0.2448364711D+01  0.3882703484D+01
 c 1.16   0.2571882731D-02  0.6627591855D-02 -0.2154576094D-01  0.4996584495D-01 -0.1432453943D+00  0.2164004986D+00 -0.5882472077D+00  0.6277827007D+00 -0.1443098299D+01  0.2427141044D+01 -0.1191806855D+01 -0.2067948985D+01  0.5999749384D+01 -0.1200699250D+02 -0.1825148246D+02  0.2601500287D+02
 P   C    178500.0000  26640.0000   6033.0000   1698.0000    548.6000    195.7000     75.8200     31.5200     13.5700      5.8950      2.5730      1.0510      0.4243      0.1681      0.0637
 c 1.15  -0.5185577263D-07  0.3276453013D-07  0.1780161036D-07 -0.2162060464D-07 -0.5376131273D-07 -0.2164853811D-03 -0.7289305999D-03 -0.3026939215D-02 -0.1107629891D-01 -0.3251571634D-01 -0.9959084162D-01 -0.2466553311D+00 -0.3835436983D+00 -0.3617647474D+00 -0.1118195279D+00
 c 1.15  -0.9490273469D-08 -0.1327648060D-07 -0.1200669922D-08  0.3213461172D-09  0.1773094571D-07 -0.3097053774D-03 -0.6899251212D-03 -0.4538897392D-02 -0.1164512101D-01 -0.4339404713D-01 -0.1066798881D+00 -0.5241045653D+00 -0.3497406427D+00  0.7433005053D+00  0.3271506281D+00
 c 1.15   0.1217368831D-07  0.1838557845D-07 -0.3106938187D-07  0.2400872644D-07  0.1112124079D-07 -0.1366166554D-03 -0.4448388040D-03 -0.1973543523D-02 -0.6914440854D-02 -0.1567320634D-01 -0.4951323142D-01 -0.4058933605D+00 -0.9419248809D-01  0.1538235915D+01 -0.1532719352D+01
 c 1.15  -0.1387261516D-02 -0.5689617440D-02 -0.1263386029D-01 -0.2723623204D-01 -0.6221575893D-01 -0.1063258393D+00 -0.2165113964D+00 -0.2395621887D+00 -0.3959879989D+00 -0.1152916005D+00 -0.3277894086D+00  0.4513970714D+00  0.1834360008D+00 -0.3736195117D+00  0.1691741402D+00
 c 1.15   0.1261848526D-02  0.1278313926D-01  0.1964117280D-01  0.4117463305D-01  0.1101486250D+00  0.1401986578D+00  0.3934502461D+00  0.8220627651D-01  0.4113239052D+00 -0.1276037307D+01  0.4594656107D+00 -0.5275091415D+00  0.1295838836D+01 -0.1154650815D+01  0.4585248471D+00
 c 1.15  -0.1486931035D-02 -0.2219919239D-03 -0.8349872156D-02 -0.4786007857D-02 -0.2074007969D-01 -0.1004544970D+00  0.2359212413D-01 -0.3092633279D+00  0.2867427962D+00 -0.7676914983D-01  0.1204517201D+01 -0.3086434544D+01  0.3677551658D+01 -0.2555218700D+01  0.9381483216D+00
 c 1.15  -0.2504419357D-02  0.1565813573D-01  0.1109868171D-01  0.1156452107D-01  0.1012110046D+00 -0.3378126215D-01  0.5109424314D+00 -0.6660193225D+00  0.8308854682D+00 -0.2717165259D+01  0.4199132839D+01 -0.3265461088D+01  0.1568334918D+01 -0.5201858225D+00  0.1152693399D+00
 D   C       195.7000     75.8200     31.5200     13.5700      5.8950      2.5730      1.0510      0.4243      0.1681      0.0637
 c 1.10  -0.1055110454D-07  0.2181112421D-07 -0.1089910672D-07 -0.2509894067D-07  0.9546900676D-02  0.4511973222D-01  0.3304897826D+00  0.5730053183D+00  0.2118266874D+00 -0.2909498841D-07
 c 1.10  -0.1394576615D-02 -0.1048891364D-02 -0.9102983694D-02 -0.9883924642D-02 -0.1857533151D-01 -0.2645470669D-01 -0.7105988693D+00 -0.1028250154D+00  0.1213892482D+01 -0.4857798170D+00
 c 1.10   0.1862312638D-02 -0.4264467556D-02  0.1273347829D-01 -0.1702448391D-01  0.5758442002D-01 -0.6223170619D-02 -0.1935505053D-01  0.3797348008D-01  0.5172174583D+00 -0.1269308079D+01
 c 1.10  -0.1398998202D-01 -0.2931950280D-01 -0.7791420038D-01 -0.1879547206D+00 -0.3441403456D+00 -0.6071105127D+00  0.1974815531D+00  0.6555894798D+00 -0.7241327076D+00  0.2563677786D+00
 F   C         5.8950      2.5730      1.0510      0.4243      0.1681
 c 1.5   0.3184211405D-01  0.9938312029D-01  0.4653028065D+00  0.5125884036D+00  0.1192780099D+00
 S   N    211000.0000  31610.0000   7190.0000   2036.0000    662.2000    234.5000     88.1300     34.7500     14.2300      6.0120      2.5390      1.0460      0.4212      0.1665      0.0578      0.0450
 c 1.16  -0.1356270685D-04 -0.1053149829D-03 -0.5546372811D-03 -0.2331793823D-02 -0.8517048587D-02 -0.2811238553D-01 -0.8202913209D-01 -0.1981274901D+00 -0.3529086079D+00 -0.3508954325D+00 -0.1099817405D+00 -0.1350942609D-01 -0.2703167980D-01 -0.1188678691D-01 -0.7388164093D-03 -0.1365093840D-06
 c 1.16  -0.3589883635D-05 -0.2822139241D-04 -0.1482976129D-03 -0.6270121550D-03 -0.2285179554D-02 -0.7658549878D-02 -0.2278428336D-01 -0.5874700988D-01 -0.1194280074D+00 -0.1732236761D+00 -0.6700422679D-01  0.2890013275D+00  0.5642959586D+00  0.2908021307D+00  0.1059479905D-01  0.9098167750D-07
 c 1.16  -0.3920078725D-05 -0.2997863417D-04 -0.1604873266D-03 -0.6641742667D-03 -0.2498782445D-02 -0.8166788229D-02 -0.2530779523D-01 -0.6521155834D-01 -0.1448137690D+00 -0.2355748510D+00 -0.7327976968D-01  0.1357605809D+01 -0.7394780610D-01 -0.1021255347D+01 -0.3130549905D-01 -0.1682872468D-06
 c 1.16  -0.4001971372D-05 -0.1669847852D-04 -0.1436127797D-03 -0.4360257211D-03 -0.2133170565D-02 -0.5429462255D-02 -0.1985201691D-01 -0.4327488695D-01 -0.1376755755D+00 -0.1798607906D+00 -0.3319929047D-01  0.2054984449D+01 -0.2793165775D+01  0.7012273034D+00  0.8402077857D+00  0.3524913664D-06
 c 1.16  -0.5894282283D-02  0.5382789469D-02 -0.1458000816D-01  0.9819154173D-02  0.5608485024D-01 -0.3382940136D-01  0.3283540175D+00 -0.8132121906D-01  0.7826989994D+00 -0.3401767583D+01  0.4877417914D+01 -0.3177938374D+01  0.5995830414D+00  0.1083505670D+00  0.4045774212D+01 -0.4263882773D+01
 c 1.16   0.5297560904D-02 -0.5344587216D-02  0.1252363250D-01 -0.1722369985D-01 -0.6450820072D-01 -0.9324135140D-02 -0.4149859693D+00 -0.2623323506D+00 -0.9945167929D+00  0.2598539209D+01 -0.1348616365D+01  0.2083165547D+00 -0.3107851690D+00  0.2041092929D+00  0.2119939544D+01 -0.2250339353D+01
 c 1.16  -0.4289957107D-02  0.2697646908D-02 -0.8573065768D-02 -0.7916288423D-02  0.5522891433D-01 -0.9349846965D-01  0.2241064679D+00 -0.3483304877D+00  0.5199242736D+00 -0.2282158952D+01  0.4738948172D+01 -0.4801137483D+01  0.2389357230D+01  0.9670843578D+00 -0.8796109979D+01  0.7729810575D+01
 P   N    211000.0000  31610.0000   7190.0000   2036.0000    662.2000    234.5000     88.1300     34.7500     14.2300      6.0120      2.5390      1.0460      0.4212      0.1665      0.0578
 c 1.15  -0.1865068208D-07 -0.8125139949D-08  0.2077621174D-07 -0.3044285902D-07  0.5709681906D-07 -0.3078878753D-03 -0.1080938599D-02 -0.5204239628D-02 -0.1846487608D-01 -0.5809795441D-01 -0.1592922577D+00 -0.3154173530D+00 -0.3923618530D+00 -0.2688414545D+00 -0.3838109096D-01
 c 1.15  -0.1367952817D-08  0.6843102710D-08 -0.5626985475D-08 -0.1109609839D-07  0.2948206162D-08 -0.4096112907D-03 -0.1578321207D-02 -0.7028922638D-02 -0.2698050187D-01 -0.7575883208D-01 -0.2799792053D+00 -0.5991439106D+00  0.2115377849D+00  0.6877905787D+00  0.9985988836D-01
 c 1.15   0.1661921769D-07 -0.1914226454D-07  0.4023439235D-07 -0.5755598171D-07  0.9360841381D-07 -0.1710186669D-03 -0.8871608860D-03 -0.2964521811D-02 -0.1475432462D-01 -0.3040515823D-01 -0.1695820954D+00 -0.3185786854D+00  0.5471652191D+00  0.5517482914D+00 -0.1238152931D+01
 c 1.15  -0.2099275929D-02 -0.5116650541D-02 -0.1621863628D-01 -0.3326294821D-01 -0.7357747838D-01 -0.1324917367D+00 -0.2531653160D+00 -0.3196260837D+00 -0.3608144872D+00 -0.9972287908D-01 -0.1344955302D+00  0.6304818272D+00 -0.3026972736D+00 -0.7365478306D-01  0.9757099190D-01
 c 1.15   0.1261096615D-02 -0.7769434399D-02  0.8891879394D-02 -0.1249625045D-01  0.2644973999D-01 -0.6763299954D-01  0.5504829531D-01 -0.3572335436D+00  0.1115204308D+00 -0.2885541380D+00  0.1981817052D+01 -0.3536514350D+01  0.3597097173D+01 -0.2361043912D+01  0.8520345189D+00
 c 1.15   0.2184115386D-03  0.2402963047D-02 -0.2923429453D-02 -0.1685235707D-02 -0.1045245777D-01  0.9628903136D-02 -0.5267106419D-01  0.1612365705D+00  0.2038788754D+00  0.2313376741D+00 -0.1554411561D+01  0.9364915064D+00  0.9992431590D+00 -0.1617852172D+01  0.8032514122D+00
 c 1.15   0.4121223487D-02  0.1665952288D-02  0.3629738331D-01  0.5401070900D-01  0.1493678960D+00  0.1794085288D+00  0.4689975518D+00  0.2015661206D-01 -0.1434723985D+00 -0.1535598748D+01  0.2053327196D+01 -0.1501364397D+01  0.1122592565D+01 -0.7385463696D+00  0.2821003056D+00
 D   N       234.5000     88.1300     34.7500     14.2300      6.0120      2.5390      1.0460      0.4212      0.1665      0.0578
 c 1.10  -0.1258333552D-07 -0.1769990799D-07  0.2677767150D-07  0.1023425168D-08  0.2181639249D-01  0.1286325244D+00  0.4891578817D+00  0.4570726734D+00  0.8344738834D-01  0.3314635253D-09
 c 1.10   0.2680497821D-02  0.1163161073D-01  0.1787980109D-01  0.7556923856D-01  0.7106013078D-01  0.3544968677D+00  0.3099804478D+00 -0.6716533401D+00 -0.1898192568D+00  0.8804086784D+00
 c 1.10  -0.3022985128D-02 -0.5958179256D-02 -0.2031945177D-01 -0.4289678520D-01 -0.8801679888D-01 -0.2266869046D+00 -0.3941179896D+00  0.2351979978D+00  0.4674531373D+00  0.4192061183D+00
 c 1.10   0.1857744405D-01  0.3533942731D-01  0.1200137921D+00  0.2452029876D+00  0.4872945875D+00  0.2968342212D+00 -0.8090776370D+00  0.1532847531D+00  0.6166883830D+00 -0.4624233696D+00
 F   N         6.0120      2.5390      1.0460      0.4212      0.1665
 c 1.5  -0.6063188734D-01 -0.2323205013D+00 -0.5670678626D+00 -0.3362368784D+00 -0.3859479727D-01
 S   O    245600.0000  36770.0000   8358.0000   2360.0000    764.2000    271.6000    103.3000     41.3900     17.2500      7.4210      3.1780      1.3380      0.5502      0.2220      0.0838      0.0700
 c 1.16  -0.1544325320D-04 -0.1200604009D-03 -0.6324558450D-03 -0.2678126092D-02 -0.9783949142D-02 -0.3170198488D-01 -0.8960472963D-01 -0.2079339512D+00 -0.3501893321D+00 -0.3181987890D+00 -0.9161228690D-01 -0.3432558855D-01 -0.6089270174D-01 -0.2881715531D-01 -0.1689386205D-02 -0.4971371125D-05
 c 1.16  -0.5309370680D-05 -0.4129910599D-04 -0.2172686677D-03 -0.9229061016D-03 -0.3376274084D-02 -0.1108208157D-01 -0.3194490994D-01 -0.7876107560D-01 -0.1508099571D+00 -0.1947046416D+00 -0.4985021909D-01  0.3111072349D+00  0.5449117142D+00  0.2735015779D+00  0.1351370483D-01  0.3732392353D-06
 c 1.16   0.4688372648D-05  0.3662618807D-04  0.1918667127D-03  0.8175152245D-03  0.2987520609D-02  0.9953015885D-02  0.2912391151D-01  0.7497890748D-01  0.1562114925D+00  0.2628821866D+00 -0.3804781678D-01 -0.1390170037D+01  0.2436716646D+00  0.9399529794D+00  0.3340557338D-01  0.5192126913D-06
 c 1.16   0.3161275917D-05  0.2760631984D-04  0.1364409301D-03  0.6282406751D-03  0.2199761174D-02  0.7475835623D-02  0.2416432756D-01  0.5411944392D-01  0.1234369631D+00  0.2469337431D+00 -0.1755803285D+00 -0.1934494529D+01  0.2974048863D+01 -0.8994315505D+00 -0.7861981663D+00 -0.8770208783D-06
 c 1.16   0.7198361978D-02  0.7735199276D+00 -0.9876435752D+00  0.1140322866D+01 -0.5638160290D+00  0.9187264510D-01  0.3868755920D-01  0.1523951401D+00  0.2948423637D-01  0.4152250163D+00 -0.1636196369D+01  0.1638949719D+01 -0.9434319138D+00  0.1720792229D+01 -0.1189543109D+02  0.1089730182D+02
 c 1.16   0.8233816755D-02  0.9042760357D+00 -0.1158215253D+01  0.1329440061D+01 -0.7005924245D+00  0.1003048981D+00 -0.2032355830D+00 -0.8399930075D-01 -0.5978759654D+00  0.6665117367D+00  0.1052994670D+01 -0.1281847243D+01 -0.4056008909D+00  0.1781503313D+01 -0.2769956887D+01  0.1597464435D+01
 c 1.16  -0.4933205749D-02 -0.5836385022D+00  0.7471818930D+00 -0.8797973593D+00  0.4502949653D+00 -0.1708312851D+00 -0.3507053045D-02 -0.4948910182D+00  0.9419939982D-01 -0.4004018433D-01  0.2045927377D+01 -0.3534684736D+01  0.2856837312D+01 -0.3410422906D+00 -0.8357519696D+01  0.7976480783D+01
 P   O    245600.0000  36770.0000   8358.0000   2360.0000    764.2000    271.6000    103.3000     41.3900     17.2500      7.4210      3.1780      1.3380      0.5502      0.2220      0.0838
 c 1.15   0.1787173710D-07  0.4745200996D-07 -0.3875209467D-07 -0.1410551121D-07 -0.2878232442D-07 -0.4051539310D-03 -0.1343703601D-02 -0.6390928267D-02 -0.2171797049D-01 -0.6736243703D-01 -0.1730481712D+00 -0.3134175361D+00 -0.3704849476D+00 -0.2609699376D+00 -0.5301314508D-01
 c 1.15   0.3176589328D-09 -0.8150257513D-08  0.1509275786D-07 -0.9008782005D-09  0.3230666200D-08 -0.5625543021D-03 -0.2079679353D-02 -0.8974708013D-02 -0.3350688321D-01 -0.9603155423D-01 -0.3336372723D+00 -0.5420130031D+00  0.2661787451D+00  0.6171236681D+00  0.1254257194D+00
 c 1.15   0.5300064147D-08 -0.8522723683D-08 -0.7136398949D-08  0.1087811681D-07 -0.1038267034D-07  0.2442250067D-03  0.1293792175D-02  0.3885821572D-02  0.2006163390D-01  0.4264600727D-01  0.2259085637D+00  0.2491644266D+00 -0.5982601568D+00 -0.5493645299D+00  0.1260434397D+01
 c 1.15  -0.1084812056D-02 -0.4328953617D-02 -0.1170888540D-01 -0.2633629208D-01 -0.5235891196D-01 -0.1149812610D+00 -0.1829377068D+00 -0.3580907648D+00 -0.3947285389D+00 -0.2832177175D+00  0.4030614977D+00  0.1337445502D+00 -0.7303947134D-02 -0.2468028252D+00  0.1694509570D+00
 c 1.15  -0.5724269418D-02 -0.1235440651D-01 -0.2778536143D-01 -0.6133437471D-01 -0.1357886387D+00 -0.2067024226D+00 -0.3669308790D+00 -0.1992341270D+00  0.1606707643D+00  0.1091520364D+01 -0.6105757141D+00 -0.7776440963D+00  0.1204584976D+01 -0.8182841722D+00  0.2878305390D+00
 c 1.15   0.3253115904D-03  0.1908620378D-02  0.2962480811D-02  0.1181098552D-01  0.1744714638D-01  0.4005666622D-01  0.9811333787D-01  0.5096594521D-01  0.3260687298D-01 -0.3732957516D-01 -0.4296199063D+00 -0.5461246054D+00  0.2425344935D+01 -0.2713796762D+01  0.1275683979D+01
 c 1.15  -0.7114406007D-02 -0.1174653223D-01 -0.2034480095D-01 -0.4858155972D-01 -0.1201064574D+00 -0.1076063047D+00 -0.3741434935D+00  0.3100707079D+00  0.3390144734D+00  0.4377100751D+00 -0.2637584634D+01  0.3686666277D+01 -0.2899428102D+01  0.1511794556D+01 -0.4586182862D+00
 D   O       271.6000    103.3000     41.3900     17.2500      7.4210      3.1780      1.3380      0.5502      0.2220      0.0838
 c 1.10   0.1473017918D-07 -0.1462501268D-07 -0.1290930677D-07  0.4611747403D-07 -0.3173706363D-01 -0.1688177706D+00 -0.5192744727D+00 -0.3944844634D+00 -0.6714399320D-01  0.4715957500D-07
 c 1.10  -0.4863717791D-02 -0.1173998932D-01 -0.3074848561D-01 -0.7767792944D-01 -0.1377258769D+00 -0.3759132848D+00 -0.3506363269D+00  0.4669142011D+00  0.4456843984D+00  0.1366206980D+00
 c 1.10   0.1574708068D-01  0.2070944233D-01  0.9647595759D-01  0.1464637758D+00  0.3358928734D+00 -0.1398133569D+00 -0.6067255129D+00  0.5606909952D+00  0.4660529726D+00 -0.1033287519D+01
 c 1.10   0.1737071095D-01  0.3642401041D-01  0.1057545925D+00  0.2388103444D+00  0.3858059471D+00  0.3254928216D+00 -0.5361121055D+00 -0.1782013636D+00  0.3847557254D+00  0.3628928220D+00
 F   O         7.4210      3.1780      1.3380      0.5502      0.2220
 c 1.5   0.8121439562D-01  0.2827095647D+00  0.5642223694D+00  0.2748790180D+00  0.2970786094D-01
 S   P   1338000.0000 199800.0000  45120.0000  12580.0000   4013.0000   1410.0000    539.5000    223.6000     99.1200     46.1800     22.3300     11.0100      5.5110      2.7950      1.4080      0.6441      0.2953      0.1292      0.0540      0.0420
 c 1.20   0.8022694940D-05  0.6310742340D-04  0.3368209355D-03  0.1459336348D-02  0.5462150911D-02  0.1806985253D-01  0.5123531078D-01  0.1202706392D+00  0.2210820592D+00  0.2790524267D+00  0.1824717678D+00  0.6287134730D-01  0.1011338891D+00  0.1611732402D+00  0.9066031436D-01  0.1181752343D-01  0.5358432762D-02  0.5068074339D-02  0.3213971231D-03  0.3194043719D-06
 c 1.20  -0.5410588035D-05 -0.4239109928D-04 -0.2261842685D-03 -0.9817495710D-03 -0.3683648743D-02 -0.1224960418D-01 -0.3522842535D-01 -0.8543751971D-01 -0.1686648356D+00 -0.2502633554D+00 -0.2231477543D+00 -0.1572587525D-01  0.2879392329D+00  0.4748250324D+00  0.2731210230D+00  0.3158304707D-01  0.4170752864D-02  0.5309525420D-02  0.1329691620D-03 -0.3810302321D-07
 c 1.20  -0.7183636211D-06 -0.5120212419D-05 -0.2732385248D-04 -0.1212486871D-03 -0.4599766641D-03 -0.1522426903D-02 -0.4481193436D-02 -0.1131305439D-01 -0.2426002090D-01 -0.4174502437D-01 -0.4603423173D-01  0.2878064491D-02  0.1093982000D+00  0.2436348062D+00  0.2611616561D+00 -0.1216986316D+00 -0.5962567645D+00 -0.4512533765D+00 -0.5158871821D-01  0.2525455578D-07
 c 1.20  -0.3800153721D-06 -0.9840007407D-05 -0.2525233608D-04 -0.1812297566D-03 -0.4960590203D-03 -0.2109932859D-02 -0.5148957591D-02 -0.1532553170D-01 -0.2814428574D-01 -0.5815694167D-01 -0.4027106324D-01 -0.2830454836D-01  0.2228941112D+00  0.1604312849D+00  0.6966074572D+00 -0.1142025541D+01 -0.1174066225D+01  0.1456065576D+01  0.2246905267D+00 -0.9680828125D-07
 c 1.20   0.8264929590D-04 -0.2090853126D-04  0.1315407009D-03  0.5275674137D-03 -0.4940820140D-03  0.5402154089D-02 -0.2351266762D-01 -0.9591611928D-03  0.4558305919D+00 -0.5111824073D-01 -0.6569112447D+00 -0.7878451426D+00  0.5464388061D+01 -0.1260173346D+02  0.1666296796D+02 -0.1564876485D+02  0.1195714476D+02 -0.6888844225D+01  0.2359960196D+01  0.4564802773D-05
 c 1.20   0.1835321978D-02 -0.4630494657D-02  0.5118973876D-02 -0.1871979662D-01  0.2052535888D-01 -0.1192505011D-01  0.1387009320D-01  0.9493504426D-01 -0.3678413757D+00  0.4714882598D+00  0.3294039313D+00  0.5265255369D+00 -0.3846291041D+01  0.4772418227D+01 -0.4684414195D+01  0.6934726734D+01 -0.7357694582D+01  0.4827915717D+01 -0.5807220383D+01  0.4384457860D+01
 c 1.20   0.8343210813D-03 -0.1328564027D-02 -0.3304381284D-02  0.9249596412D-02  0.5255509025D-02 -0.2258589074D-01  0.1312070550D-01 -0.5543714541D-01  0.2073056095D+00 -0.6080925996D-01  0.2166374373D+00 -0.3828778049D+00  0.5584785644D+00 -0.3176501974D+01  0.5657789694D+01 -0.4177354937D+01  0.5307597809D+00  0.1287713727D+01  0.2537274926D+01 -0.3521278327D+01
 c 1.20  -0.3672460123D-02  0.9162230497D-02 -0.9853494214D-02  0.3852108619D-01 -0.2135442918D-01 -0.7552134241D-02  0.8283215297D-01 -0.2773407525D+00  0.1158140225D+01 -0.1204701381D+01  0.3522433657D+00 -0.2251539637D+01  0.7548548178D+01 -0.1096896732D+02  0.8598485891D+01 -0.4845647817D+01  0.4839278004D+01 -0.7752228930D+01  0.1668763781D+02 -0.1203024848D+02
 c 1.20  -0.1517092779D-02  0.3682583492D-02  0.8000410978D-03  0.1101993282D-01 -0.3973409078D-02  0.7685851225D-01  0.1236802385D+00  0.3101145710D+00  0.3952917417D+00  0.1411731785D+00 -0.7292033059D+00 -0.9060249908D+00 -0.7334170242D+00  0.4833139512D+01 -0.5369307341D+01  0.2959710776D+01 -0.9034087005D+00 -0.1235466841D+00  0.6902377406D+00 -0.5092672741D+00
 P   P   1338000.0000 199800.0000  45120.0000  12580.0000   4013.0000   1410.0000    539.5000    223.6000     99.1200     46.1800     22.3300     11.0100      5.5110      2.7950      1.4080      0.6441      0.2953      0.1292      0.0540
 c 1.19   0.1303394007D-07 -0.4612681810D-08  0.2202996976D-07 -0.9835951063D-08  0.5064876602D-04  0.2168005757D-03  0.1122363380D-02  0.4444447514D-02  0.1536695306D-01  0.4465810656D-01  0.1104160363D+00  0.2140726864D+00  0.3066458649D+00  0.3046802525D+00  0.1673608251D+00  0.3970557238D-01  0.2431553613D-01  0.2524767657D-01  0.7561746941D-02
 c 1.19  -0.3806536439D-08  0.3347719404D-07 -0.3736182060D-07  0.3154589245D-07  0.1560396235D-04  0.6347984495D-04  0.3401370413D-03  0.1336398239D-02  0.4639704341D-02  0.1364488716D-01  0.3414432161D-01  0.6776901481D-01  0.9824109923D-01  0.1063999262D+00  0.3188574853D-01 -0.1931484457D+00 -0.4168691326D+00 -0.4124642224D+00 -0.1300016821D+00
 c 1.19   0.3210986957D-08  0.1393348162D-07  0.1734528869D-07 -0.5099036629D-08  0.2143165839D-04  0.4286407425D-04  0.4155962239D-03  0.1193210784D-02  0.5228139044D-02  0.1293993789D-01  0.3783542664D-01  0.6685007854D-01  0.1142144277D+00  0.9406137183D-01  0.1146651786D+00 -0.6923452476D+00 -0.5927732918D+00  0.7975044155D+00  0.3817657507D+00
 c 1.19   0.2501839544D-07 -0.7071354037D-08 -0.1509607409D-07 -0.1620555513D-07 -0.4528618602D-04  0.1334325025D-03  0.9265968008D-04  0.1352297382D-02  0.2270017305D-02  0.6987406466D-02  0.2744232917D-01  0.4138668864D-01  0.9003067770D-01  0.4446639646D-01  0.1769929229D+00 -0.1017965625D+01  0.1844619871D+00  0.1686721513D+01 -0.1614849662D+01
 c 1.19  -0.5824563273D-02 -0.1469272513D-02 -0.1779503316D-01 -0.2509387184D-01 -0.7341620869D-01 -0.1141355296D+00 -0.2207137222D+00 -0.2688933641D+00 -0.5084292140D+00 -0.8848235946D-01  0.4535817554D-02  0.4648100064D+00 -0.7826745218D+00  0.1159857469D+01 -0.1076480732D+01  0.9792542715D+00 -0.9104157732D+00  0.5998227691D+00 -0.2206387336D+00
 c 1.19  -0.2627695031D-01  0.1245357875D-01  0.4420456376D-02  0.1150825285D-01  0.6664962407D-01  0.5933812620D-01  0.3396928214D+00  0.3004119611D+00 -0.1012801138D+01  0.2161222557D+00  0.6587553406D+00  0.1107789366D+01 -0.3930152836D+01  0.5764349503D+01 -0.6335545606D+01  0.5977774064D+01 -0.4752683040D+01  0.2742040434D+01 -0.9371869199D+00
 c 1.19  -0.4578723889D-02  0.2920741222D-02 -0.2147218214D-01  0.1983369652D-02 -0.8108679103D-01 -0.3109344905D-01 -0.2003202179D+00 -0.3148712049D-01 -0.8779509727D-01  0.6075983617D+00  0.6123313311D-01  0.8064628731D-01 -0.1983624835D+01  0.1573545300D+01  0.6398350374D+00 -0.5585469180D+00 -0.6733465130D+00  0.9698978444D+00 -0.4579165819D+00
 c 1.19  -0.6614402565D-02 -0.3679177212D-01  0.5702160736D-01 -0.7697619545D-01  0.2144642977D+00 -0.1412625508D+00  0.6670372972D+00 -0.2222518997D+00 -0.3458326503D+00 -0.1060059524D+01  0.2801933718D+01 -0.2931325940D+01  0.1933875197D+01 -0.1986768354D+01  0.3474251717D+01 -0.4775820865D+01  0.4544116482D+01 -0.2868158475D+01  0.1025294238D+01
 c 1.19   0.1704188234D-01 -0.3634742792D-01  0.6469482032D-01 -0.8632267925D-01  0.1944921406D+00 -0.1678420103D+00  0.4468652582D+00 -0.4103763858D+00  0.6091817384D+00 -0.1531660461D+01  0.2037445931D+01 -0.2704018230D+01  0.5504403441D+01 -0.8603479927D+01  0.7714453657D+01 -0.3825872909D+01  0.8106752623D+00  0.3576576444D+00 -0.2809262088D+00
 c 1.19   0.2184061812D-02 -0.9486941167D-02 -0.8218007733D-02 -0.3139324759D-01 -0.4829090546D-01 -0.1167888870D+00 -0.1640066455D+00 -0.2478406358D+00  0.6160714708D-01  0.2028623361D+00  0.7571628251D+00 -0.1571954927D+00  0.3704593981D+00 -0.1476659905D+01  0.1196515995D+01 -0.1286344666D+01  0.1694395763D+01 -0.1328807448D+01  0.5298102300D+00
 D   P      4013.0000   1410.0000    539.5000    223.6000     99.1200     46.1800     22.3300     11.0100      5.5110      2.7950      1.4080      0.6441      0.2953      0.1292      0.0540
 c 1.15  -0.7629635042D-08  0.1144496419D-07  0.1334503538D-07 -0.4402604913D-07  0.2485150507D-07  0.1698987764D-07 -0.2271000588D-07  0.4885212634D-02  0.5472609567D-02  0.1856664026D-01  0.4759149284D-01  0.3366550506D+00  0.5287999809D+00  0.2171624215D+00  0.5759655956D-08
 c 1.15   0.7570542158D-03  0.4551963021D-02  0.1087438200D-01  0.3192899692D-01  0.6729891698D-01  0.1352585792D+00  0.2334337751D+00  0.3057445504D+00  0.3096308189D+00  0.1852072197D+00  0.8847408246D-01 -0.1018128655D+00 -0.9309321382D-01  0.3079633559D-01 -0.4536882281D-01
 c 1.15   0.5315265602D-02 -0.2242201088D-02  0.7276876052D-02  0.3979035112D-02  0.3610925173D-01  0.7009522829D-01  0.1663268503D-01  0.4522985616D-01 -0.1173624924D+00 -0.9496681608D-01 -0.3297758680D+00  0.1430339885D+01 -0.5064497209D+00 -0.1054423522D+01  0.6934620627D+00
 c 1.15  -0.7333452526D-02  0.8212411194D-02 -0.1071944609D-01  0.1809663657D-01 -0.3249165611D-01 -0.1173995851D-01 -0.1052120222D-01 -0.5214191995D-02  0.3848564564D-02  0.8085805967D-02  0.2888186590D-01 -0.1837254416D+00  0.6174478195D+00 -0.1195988498D+00 -0.1009712837D+01
 c 1.15  -0.9209311381D-02  0.2538557678D-01  0.3728520841D-02  0.9913341105D-01  0.9986034374D-01  0.2432044501D+00  0.3104911877D+00  0.1560188556D+00 -0.4421256378D-01 -0.8691114353D+00 -0.5431627510D-01  0.4751251207D+00 -0.4789682072D+00  0.5997571786D+00 -0.3138740948D+00
 F   P        11.0100      5.5110      2.7950      1.4080      0.6441      0.2953      0.1292
 c 1.7   0.2684501834D-01  0.2127745384D-01  0.5139140347D-01  0.9352993138D-01  0.4474429005D+00  0.4758781313D+00  0.1292773840D+00
 }

